Integrated Optimization of Power Split, Engine Thermal Management, and Cabin Heating for Hybrid Electric Vehicles

Cabin heating demand and engine efficiency degradation in cold weather lead to considerable increase in fuel consumption of hybrid electric vehicles (HEVs), especially in congested traffic conditions. This paper presents an integrated power and thermal management (i-PTM) scheme for the optimization of power split, engine thermal management, and cabin heating of HEVs. A control-oriented model of a power split HEV, including power and thermal loops, is developed and experimentally validated against data collected from a 2017 Toyota Prius HEV. Based on this model, the dynamic programming (DP) technique is adopted to derive a bench-mark for minimal fuel consumption, using 2-dimensional (power split and engine thermal management) and 3-dimensional (power split, engine thermal management, and cabin heating) formulations. Simulation results for a real-world congested driving cycle show that the engine thermal effect and the cabin heating requirement can significantly influence the optimal behavior for the power management, and substantial potential on fuel saving can be achieved by the i-PTM optimization as compared to conventional power and thermal management strategies.

==> ref <==
@article{zhao2017accelerated,
  title={Accelerated evaluation of automated vehicles safety in lane-change scenarios based on importance sampling techniques},
  author={Zhao, Ding and Lam, Henry and Peng, Huei and Bao, Shan and LeBlanc, David J and Nobukawa, Kazutoshi and Pan, Christopher S},
  journal={IEEE transactions on intelligent transportation systems},
  volume={18},
  number={3},
  pages={595--607},
  year={2017},
  publisher={IEEE}
}


%************************************************
@article{Cao2017,
author = {Cao, Peng and Hu, Yubai and Miwa, Tomio and Wakita, Yukiko and Morikawa, Takayuki and Liu, Xiaobo},
journal = {Journal of Intelligent Transportation Systems},
number = {4},
pages = {271--284},
publisher = {Taylor {\&} Francis},
title = {{An optimal mandatory lane change decision model for autonomous vehicles in urban arterials}},
volume = {21},
year = {2017}
}

%************************************************
@article{Rios-Torres2017,
author = {Rios-Torres, Jackeline and Malikopoulos, Andreas A.},
doi = {10.1109/TITS.2016.2587582},
journal = {IEEE Transactions on Intelligent Transportation Systems},
number = {4},
pages = {780--789},
title = {{Automated and Cooperative Vehicle Merging at Highway On-Ramps}},
volume = {18},
year = {2017}
}
%****************************************************
@article{Wan2011,
author = {Wan, Liming and Raksincharoensak, Pongsathorn and Maeda, Kozo and Nagai, Masao},
journal = {International Journal of Automotive Engineering},
pages = {7--12},
title = {{Lane Change Behavior Modeling for Autonomous Vehicles Based on Surroundings Recognition}},
volume = {2},
year = {2011}
}
%**********************************************************
@article{Ulbrich2015,
author = {Ulbrich, Simon and Maurer, Markus},
doi = {10.1109/ITSC.2015.165},
journal = {IEEE Conference on Intelligent Transportation Systems, Proceedings, ITSC},
pages = {989--995},
title = {{Towards Tactical Lane Change Behavior Planning for Automated Vehicles}},
volume = {2015-Octob},
year = {2015}
}

%********************************************************************
@article{Kuwata2009,
author = {Kuwata, Yoshiaki and Teo, Justin and Fiore, Gaston and Karaman, Sertac and Frazzoli, Emilio and How, Jonathan P},
number = {5},
pages = {1105--1118},
title = {{Real-Time Motion Planning With Applications to Autonomous Urban Driving}},
volume = {17},
year = {2009}
}
%******************************************************************
@article{Naranjo2008,
doi = {10.1109/TITS.2008.922880},
journal = {IEEE Transactions on Intelligent Transportation Systems},
keywords = {Fuzzy control,Hybrid control,Intelligent control,Proportional-integral differential (PID) control,Road vehicle control},
number = {3},
pages = {438--450},
title = {{Lane-change fuzzy control in autonomous vehicles for the overtaking maneuver}},
volume = {9},
year = {2008}
}
%****************************************************************
@article{Division1986,
author = {Division, Gipps},
number = {5},
title = {{Lane-Changing decisions}},
volume = {20},
year = {1986}
}

%*****************************************************************

@article{Kesting2007,
author = {Kesting, Arne},
title = {{MOBIL : General Lane-Changing Model for Car-Following Models}},
year = {2007}
}

%*******************************************************************8
@article{Toledo2007,
author = {Toledo, Tomer and Koutsopoulos, Haris N. and Ben-Akiva, Moshe},
doi = {10.1016/j.trc.2007.02.002},
journal = {Transportation Research Part C: Emerging Technologies},
number = {2},
pages = {96--112},
pmid = {1051786},
title = {{Integrated driving behavior modeling}},
volume = {15},
year = {2007}
}
%*********************************************************************
@article{Hunt1994,
author = {Hunt, J. G. and Lyons, G. D.},
doi = {10.1016/0968-090X(94)90012-4},
journal = {Transportation Research Part C},
number = {4},
pages = {231--245},
title = {{Modelling dual carriageway lane changing using neural networks}},
volume = {2},
year = {1994}
}

%*********************************************************************
@article{Wu2003,
author = {Wu, J. and Brackstone, M. and McDonald, M.},
doi = {},
journal = {Transportation Research Part C},
number = {1},
pages = {463--479},
title = {{The validation of a microscopic simulation model: a methodological case study}},
volume = {116},
year = {2003}
}

%*********************************************************************
@article{Toledo2009,
author = {Toledo, Tomer and Katz, Romina},
doi = {10.3141/2124-08},
journal = {Transportation Research Record: Journal of the Transportation Research Board},
pages = {81--88},
title = {{State Dependence in Lane-Changing Models}},
volume = {2124},
year = {2009}
}
%*********************************************************************
@article{Motamedidehkordi2017,
author = {Motamedidehkordi, N and Amini, S and Hoffmann, S and Busch, F and Fitriyanti, M R},
doi = {10.1109/MTITS.2017.8005678},
journal = {2017 5th IEEE International Conference on Models and Technologies for Intelligent Transportation Systems (MT-ITS)},
pages = {268--273},
title = {{Modeling tactical lane-change behavior for automated vehicles: A supervised machine learning approach}},
year = {2017}
}

%************************************8
@article{Division1986,
author = {Division, Gipps},
number = {5},
title = {{A model for the structure of lane-changing decisions}},
journal = {Transpn. Res-B},
volume = {20},
year = {1986},
pages = {403--414}
}
%--------------------------------------------------------
@article{Guo2016,
author = {Guo, Lulu and Gao, Bingzhao and Gao, Ying and Chen, Hong},
doi = {10.1109/TITS.2016.2634019},
journal = {IEEE Transactions on Intelligent Transportation Systems},
number = {8},
pages = {2153--2162},
title = {{Optimal Energy Management for HEVs in Eco-Driving Applications Using Bi-Level MPC}},
volume = {18},
year = {2016}
}
%----------------------------------------------------------
@article{Kamal2011,
author = {Kamal, M. A S and Mukai, Masakazu and Murata, Junichi and Kawabe, Taketoshi},
doi = {10.1109/TITS.2011.2112648},
isbn = {1524-9050},
issn = {15249050},
journal = {IEEE Transactions on Intelligent Transportation Systems},
keywords = {Driver-assistance system,eco-driving,model predictive control},
number = {3},
pages = {783--794},
title = {{Ecological vehicle control on roads with up-down slopes}},
volume = {12},
year = {2011}
}

%----------------------------------------------------------
@article{Rios-Torres2017,
author = {Rios-Torres, Jackeline and Malikopoulos, Andreas A.},
doi = {10.1109/TITS.2016.2587582},
journal = {IEEE Transactions on Intelligent Transportation Systems},
number = {4},
pages = {780--789},
title = {{Automated and Cooperative Vehicle Merging at Highway On-Ramps}},
volume = {18},
year = {2017}
}

%----------------------------------------------------------
@article{Ahmed1999,
author = {Ahmed, K. I.},
doi = {},
journal = {Massachusetts Institute of Technology, Master of Science},
number = {},
pages = {1-189},
title = {{Modeling drivers' acceleration and lane changing behavior}},
volume = {},
year = {1999}
}

%-----------------------------------------------------------
@article{Moridpour2010,
author = {Moridpour, Sara and Sarvi, Majid and Rose, Geoff},
doi = {10.3328/TL.2010.02.03.157-173},
journal = {Transportation Letters},
keywords = {drivers,lane changing maneuvers,lane changing models},
number = {3},
pages = {157--173},
title = {{Lane changing models: a critical review}},
volume = {2},
year = {2010}
}

%------------------------------------------------------------
@article{Jula2000,
author = {Jula, Hossein and Kosmatopoulos, Elias B. and Ioannou, Petros A.},
doi = {10.1109/25.901899},
journal = {IEEE Transactions on Vehicular Technology},
number = {6},
pages = {2295--2308},
title = {{Collision avoidance analysis for lane changing and merging}},
volume = {49},
year = {2000}
}

%--------------------------------------------------------------
@article{Hidas2005,
author = {Hidas, Peter},
doi = {10.1016/j.trc.2004.12.003},
journal = {Transportation Research Part C: Emerging Technologies},
keywords = {Agents,Lane changing,Merging,Micro-simulation},
number = {1},
pages = {37--62},
title = {{Modelling vehicle interactions in microscopic simulation of merging and weaving}},
volume = {13},
year = {2005}
}

%--------------------------------------------------------------
@article{Sciarretta2015,
author = {Sciarretta, A. and De Nunzio, G. and Ojeda,L.},
doi = {},
journal = {IEEE Control system magazine},
keywords = {},
number = {},
pages = {},
title = {{Optimal Eco-driving control}},
volume = {},
year = {2015}
}

%--------------------------------------------------------
@article{Barth2009,
author = {Barth, Matthew and Boriboonsomsin, Kanok},
doi = {10.1016/j.trd.2009.01.004},
journal = {Transportation Research Part D: Transport and Environment},
keywords = {Eco-driving,Intelligent speed adaptation,Intelligent transportation systems,Telematics},
number = {6},
pages = {400--410},
publisher = {Elsevier Ltd},
title = {{Energy and emissions impacts of a freeway-based dynamic eco-driving system}},
url = {http://dx.doi.org/10.1016/j.trd.2009.01.004},
volume = {14},
year = {2009}
}

%---------------------------------------------------------
@article{Yang2010,
author = {Yang, H. H. and Peng, H.},
doi = {10.1080/00423110903128524},
journal = {Vehicle System Dynamics},
keywords = {Active safety,Car-following,Driver errors,Driver model},
number = {6},
pages = {751--773},
title = {{Development of an errorable car-following driver model}},
volume = {48},
year = {2010}
}

%-------------------------------------------------------
@article{Zhao2016,
author = {Zhao, D and Peng, H and Bao, S and Nobukawa, K and LeBlanc, D and Pan, C},
doi = {10.1201/b21185-33},
journal = {The Dynamics of Vehicles on Roads and Tracks},
number = {Litman},
pages = {287--296},
title = {{Accelerated evaluation of automated vehicles using extracted naturalistic driving data}},
year = {2016}
}

@article{Arsie10,
author = {Ivan Arsie and Rizzo, Gianfranco and Sorrentino, Marco},
doi = {10.1016/j.conengprac.2010.01.015},
journal = {Control Engineering Practice},
number = {11},
pages = {1231--1238},
publisher = {Elsevier},
title = {{Effects of engine thermal transients on the energy management of series hybrid solar vehicles}},
volume = {18},
year = {2010}
}


@article{Kessels08,
author = {Kessel, J and Foster, D and Bleuanus, W},
journal = {in Proc of the International Conference on Advances in Hybrid Powertrains},
number = {},
pages = {1-6},
publisher = {},
title = {{Towards integrated powertrain control: thermal management of NG heated catalyst system}},
volume = {},
year = {2008}
}


@article{Gissing2016,
author = {Gissing, Jorg and Themann, Philipp and Baltzer, Sidney and Lichius, Thomas and Eckstein, Lutz},
doi = {10.1109/TCST.2015.2468055},
journal = {IEEE Transactions on Control Systems Technology},
number = {3},
pages = {1126--1133},
title = {{Optimal Control of Series Plug-In Hybrid Electric Vehicles Considering the Cabin Heat Demand}},
volume = {24},
year = {2016}
}

@article{Shams-Zahraei2012,
author = {Shams-Zahraei, Mojtaba and Kouzani, Abbas Z. and Kutter, Steffen and B{\"{a}}ker, Bernard},
doi = {10.1016/j.jpowsour.2012.05.055},
journal = {Journal of Power Sources},
pages = {237--248},
title = {{Integrated thermal and energy management of plug-in hybrid electric vehicles}},
volume = {216},
year = {2012}
}

@article{Sciarretta2007,
author = {Sciarretta, A. and Guzzella, L.},
doi = {10.1109/MCS.2007.338280},
journal = {IEEE Control Systems},
number = {2},
pages = {60--70},
title = {{Control of hybrid electric vehicles}},
volume = {27},
year = {2007}
}

@article{haowang2018,
author = {Wang, H. and Kolmanovsky, I. and Amini,  M. R. and Sun, J.},
doi = {10.1109/MCS.2007.338280},
journal = {Proceedings of American Control Conference},
number = {},
pages = {828--833},
title = {{Model Predictive Climate Control of Connected and Automated Vehicles for Improved Energy Efficiency}},
volume = {},
year = {2018}
}


@article{Lin2003,
author = {Lin, Chan-Chiao and Peng, Huei and Grizzle, J W and Kang, Jun-Mo},
doi = {10.1109/TCST.2003.815606},
journal = {IEEE Transactions on Control Systems Technology},
number = {6},
pages = {839--849},
title = {{Power management strategy for a parallel hybrid electric truck}},
volume = {11},
year = {2003}
}

@article{Lin2004,
author = {Lin, Chan-Chiao and Peng, Huei and Grizzle, J W},
journal = {Proceedings of the American Control Conference},
pages = {4710--4715},
title = {{A Stochastic Control Strategy for Hybrid Electric Vehicles}},
year = {2004}
}

@article{Kim2010,
author = {Kim, Namwook and Cha, Sukwon and Peng, Huei},
journal = {IEEE Transactions on Control Systems Technology},
number = {5},
pages = {1279--1287},
title = {{Optimal Control of Hybrid Electric Vehicles Based on Pontryagin's Minimum Principle}},
volume = {19},
year = {2010}
}

@article{Serrao2009,
author = {Serrao, Lorenzo and Onori, Simona and Rizzoni, Giorgio},
doi = {10.1109/ACC.2009.5160628},
journal = {Proceedings of the American Control Conference},
pages = {3964--3969},
title = {{ECMS as a realization of pontryagin's minimum principle for HEV control}},
year = {2009}
}

@article{LiuTeng2017,
author = {Liu, Teng and Hu, Xiaosong and Li, Shengbo and Cao, Dongpu},
doi = {10.1109/TMECH.2017.2707338},
journal = {IEEE/ASME Transactions on Mechatronics},
number = {c},
pages = {1--1},
title = {{Reinforcement Learning Optimized Look-Ahead Energy Management of a Parallel Hybrid Electric Vehicle}},
volume = {4435},
year = {2017}
}

@article{Zou2016,
author = {Zou, Yuan and Liu, Teng and Liu, Dexing and Sun, Fengchun},
doi = {10.1016/j.apenergy.2016.03.082},
journal = {Applied Energy},
pages = {372--382},
publisher = {Elsevier Ltd},
title = {{Reinforcement learning-based real-time energy management for a hybrid tracked vehicle}},
volume = {171},
year = {2016}
}

@article{Borhan2012,
author = {Borhan, Hoseinali and Member, Student and Vahidi, Ardalan and Phillips, Anthony M and Kuang, Ming L and Kolmanovsky, Ilya V and Cairano, Stefano Di},
journal = {IEEE Transactions on Control Systems Technology},
number = {3},
pages = {593--603},
title = {{MPC-Based Energy Management of a Power-Split Hybrid Electric Vehicle}},
volume = {20},
year = {2012}
}

@article{Cairano2014,
author = {Cairano, Stefano Di and Bernardini, Daniele and Bemporad, Alberto and Kolmanovsky, Ilya V.},
doi = {10.1109/TCST.2013.2272179},
journal = {IEEE Transactions on Control Systems Technology},
number = {3},
pages = {1018--1031},
title = {{Stochastic MPC with learning for driver-predictive vehicle control and its application to HEV energy management}},
volume = {22},
year = {2014}
}


@article{LiuJinm2008,
author = {Liu, Jinming and Peng, Huei},
journal = {IEEE Transactions on Control Systems Technology},
number = {6},
pages = {1242--1251},
title = {{Modeling and Control of a Power-Split Hybrid Vehicle}},
volume = {16},
year = {2008}
}

@article{Kim2014,
author = {Kim, Namwook and Rousseau, Aymeric and Lee, Daeheung and Lohse-busch, Henning},
doi = {10.4271/2014-01-1784.Abstract},
journal = {SAE Technical Paper},
number = {2014-01-1784},
pages = {1--10},
title = {{Thermal model development and validation for 2010 Toyota Prius}},
year = {2014}
}

@article{Hu2012,
author = {Hu, Xiaosong and Li, Shengbo and Peng, Huei},
doi = {10.1016/j.jpowsour.2011.10.013},
journal = {Journal of Power Sources},
pages = {359--367},
publisher = {Elsevier B.V.},
title = {{A comparative study of equivalent circuit models for Li-ion batteries}},
volume = {198},
year = {2012}
}

@article{Berteskas1995,
author = {Bertsekas, D P},
journal = {Belmont, MA: Athena Scientific},
title = {{Dynamic Programming and Optimal Control}},
year = {1995}
}


@article{Sun2015,
author = {Sun, Chao and Moura, Scott Jason and Hu, Xiaosong and Hedrick, J. Karl and Sun, Fengchun},
doi = {10.1109/TCST.2014.2361294},
journal = {IEEE Transactions on Control Systems Technology},
number = {3},
pages = {1075--1086},
title = {{Dynamic Traffic Feedback Data Enabled Energy Management in Plug-in Hybrid Electric Vehicles}},
volume = {23},
year = {2015}
}

@article{Liujinm2005,
author = {Liu, Jinming and Peng, Huei and Filipi, Zoran},
journal = {Proceedings of the American Control Conference},
pages = {24--28},
title = {{Modeling and Analysis of the Toyota Hybrid System}},
year = {2005}
}

@article{MarinaMartinez2016,
author = {{Marina Martinez}, Clara and Hu, Xiaosong and Cao, Dongpu and Velenis, Efstathios and Gao, Bo and Wellers, Matthias},
doi = {10.1109/TVT.2016.2582721},
journal = {IEEE Transactions on Vehicular Technology},
number = {6},
pages = {4534--4549},
title = {{Energy Management in Plug-in Hybrid Electric Vehicles: Recent Progress and a Connected Vehicles Perspective}},
volume = {66},
year = {2016}
}

@article{Silvas2017,
author = {Silvas, Emilia and Hofman, Theo and Murgovski, Nikolce and Etman, L F Pascal and Steinbuch, Maarten},
journal = {IEEE Transactions on Vehicular Technology},
number = {1},
pages = {57--70},
title = {{Review of Optimization Strategies for System-Level Design in Hybrid Electric Vehicles}},
volume = {66},
year = {2017}
}

@article{Tashiro2016,
author = {Tashiro, Tsutomu},
journal = {8th IFAC Symposium on Advances in Automotive Control},
keywords = {Automotive control,Fuel efficiency,Hybrid electric vehicle,Power management,Prediction method},
number = {11},
pages = {393--398},
title = {{Power Management of a Hybrid Electric Vehicle During Warm-up Period Considering Energy Consumption of Cabin Heat Components}},
volume = {49},
year = {2016}
}

@article{Engbroks2018,
author = {Engbroks, Lukas and Gorke, Daniel and Schmiedler, Stefan and Strenkert, Jochen and Geringer, Bernhard},
title = {{Applying forward dynamic programming to combined energy and thermal management optimization of hybrid electric vehicles}},
journal = {5th IFAC Conference on Engine and Powertrain Control Simulation and Modeling},
pages = {416--422},
year = {2018}
}



























